Safety Assurances for Human-Robot Interaction via Confidence-aware Game-theoretic Human Models

An outstanding challenge with safety methods for human-robot interaction is reducing their conservatism while maintaining robustness to variations in human behavior. In this work, we propose that robots use confidence-aware game-theoretic models of human behavior when assessing the safety of a human-robot interaction. By treating the influence between the human and robot as well as the human's rationality as unobserved latent states, we succinctly infer the degree to which a human is following the game-theoretic interaction model. We leverage this model to restrict the set of feasible human controls during safety verification, enabling the robot to confidently modulate the conservatism of its safety monitor online. Evaluations in simulated human-robot scenarios and ablation studies demonstrate that imbuing safety monitors with confidence-aware game-theoretic models enables both safe and efficient human-robot interaction. Moreover, evaluations with real traffic data show that our safety monitor is less conservative than traditional safety methods in real human driving scenarios.

==> introv1.tex <==
\section{Introduction}
In highly dynamic human-robot interactions like the ones found in autonomous driving, assessing if a robot is safe around nearby humans is critical yet challenging. For example, consider a robot car that is merging into a round-about with an oncoming human-driven car (Fig.~\ref{fig:front_fig}). Assessing if the robot is on the verge of collision with the human-driven car depends not only on the current state, but also the possible future behaviors of the human and robot as they move through the scene. 
% here safe means not on the verge of collision

Forward reachability methods have been used to compute the set of states where other agents could be in the future \cite{althoff2011set, liu2017provably}, after which the robot plans to avoid this set. While safe, these methods often lead to overly-conservative robot behaviors especially in close-proximity interactive scenarios (e.g., merging or lane-changing). Prior work \cite{driggs2018robust, bajcsy2020robust} leveraged structure in human decision-making to obtain data-driven restrictions on human actions and, ultimately, their forward reachable set but are unable to capture safety-critical interaction effects between the human and robot. 

Alternatively, zero-sum differential games \cite{mitchell2005time, margellos2011hamilton, dhinakaran2017hybrid, leung2020infusing} have been used to develop \textit{safety monitors} which quantify the safety (i.e., proximity to inevitable collision) of the joint human-robot system.
% provide strong safety assurances for robots acting around other agents in safety-critical situations. 
To ensure robustness to all---including worst-case---human behavior in such safety-critical scenarios, the human is modelled as an adversary who chooses their behavior from the set of all dynamically-feasibly control signals. While generally less conservative than full forward reachability, this approach still often suffers from falsely flagging safe states as unsafe because of the full control authority and adversarial nature of the human model. Recent work has attempted to reduce this conservatism by leveraging data-driven human trajectory forecasts to restrict the set of feasible human controls used during the safety computation \cite{li2020prediction}. However, this approach blindly trusts the set of feasible human controls generated by the data-driven predictor; if the quality of the data-driven forecasts degrade, this method is unable to safeguard against these errors, compromising the safety monitor.
% These approaches are good because they reduce conservatism and adapt through data, but (a) these models treat the human as acting in isolation and (b) challenging to monitor confidence in the model.

Ultimately, when reducing the conservatism of the robot's safety assurances, existing methods have (a) focused exclusively on human behavior models which treat the \textit{human as acting in isolation} and (b) been unable to monitor the \textit{confidence} in their restrictions. 

In this paper, we propose that robots should leverage insights from cognitive science research and utilize theory of mind models of human decision-making \cite{baker2014modeling, carruthers1996theories, gergely2003teleological, sodian2004infants} in their safety monitors. 
Specifically, we leverage a subclass of theory of mind models---Stackelberg games \cite{von2010market}---which are well-suited to capture naturally-emergent leader-follower behavior in human-robot coordination scenarios such as merging, lane-switching, or intersection maneuvers.  
We extend existing work on leader-follower games \cite{sadigh2016planning, fisac2019hierarchical, schwarting2019social} by not assuming \textit{a priori} which role the human takes in the interaction, and instead enable robots to infer the role of the human in a dynamic interaction. 
% but these typically model the human as an optimal follower in the interaction. 
%  we propose that robots should estimate the degree to which humans abide by \textit{leader-follower roles} and reduce the conservatism of their safety assurances accordingly.

Importantly, we also recognize that the safety of the overall human-robot system hinges on fact that the interaction actually exhibits this leader-follower influence at all---if this model is misspecified, the safety guarantee can be compromised.
Thus, we also propose that the robot monitor it's \textit{confidence} in the leader-follower behavior model. To do this, we extend existing work on model confidence estimation \cite{fisac2018probabilistically, bobu2020quantifying} to the game-theoretic domain. 
When the robot jointly infers the human's role in the game along with model confidence, the robot naturally reduces conservatism in its safety monitor when it detects emergent leader-follower interactions; on the other hand, when the observed human behavior cannot be well-explained by the interaction model, the robot automatically shifts to safeguarding against worst-case game-theoretic human behavior. 
% leader-follower inference is coupled with confidence estimation
% \item In reality, there is \textit{influence} between the human and robot. 
% \item Such models of the human-robot interaction have been investigated in the context of planning and prediction\cite{sadigh2016planning, fisac2019hierarchical, schwarting2019social}, but these typically model the human as an optimal follower in the interaction. 
% \item In reality, the robot needs to safeguard against the possibility that the human takes the leader role too. \abnote{need to diversify the citations -- cite Forrest/DFK, Mac Schwager, maybe something from Lillian Ratliff or ?}
    
Through a range of simulated human behavior models and real traffic data at a roundabout and highway, we demonstrate that confidence-aware role inference can effectively enable robots to modulate the conservatism of their safety monitors when engaging in dynamic interactions with humans. 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{media/front_fig.jpg}
    \caption{Robot car (white) merges into a round-about with a nearby human-driven car (orange). (left) Human behaves as a leader, but the robot protects against the full backwards reachable tube (BRT), making it overly-conservative. (center) Our Bayesian BRT infers that the human is a leader and shrinks the unsafe states accordingly. (right) When the human does not behave according to the model, the robot detects this and automatically reverts to the full BRT.}
    \label{fig:front_fig}
    \vspace{-2em}
\end{figure}

% \section{Related Work}
% \abnote{we could actually combine related work with intro to save space...}
% \noindent\textbf{Safety-critical control around humans.}
% \begin{itemize}
%     \item Full forward reachable set: safe but too conservative to safeguard against. Thus, there are methods for restricting FRS \cite{driggs2018robust, bajcsy2020robust}, but these don't capture interaction between agents and still possibly too conservative...
%     \item BRT's: less conservative under the game-theoretic assumption \cite{mitchell2005time, leung2020infusing}.
% \end{itemize}

% \noindent \textbf{Structured human decision-making models.}
% \begin{itemize}
%     \item Data-driven human behavior models \cite{li2020prediction} [Liting, Mo's paper, Mathias’s stuff]
%     \item the above approaches are good because they reduce conservatism and adapt through data, but (a) these models treat the human as acting in isolation and (b) challenging to monitor confidence in the model.
%     \item theory of mind game theory stuff [Jaime, Dorsa, social behavior for autonomous vehicles paper], but these all assume that the robot is the leader and the human is follower. This may not hold in practice, and we need robot to infer if the human is taking the lead instead.
% \end{itemize}

==> results.tex <==



\begin{figure}[ht]
\begin{center}
\begin{picture}(300, 350)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% left side

\put(25, 200){\epsfig{file=media/simulated_human/simulated_confident_follower_test_1_safe_control_ourBRT1.png, width = 0.42\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
\put(0,  250){\epsfig{file=media/simulated_human/simulated_confident_follower_test_1_safe_control_ourBRT_latent_state1.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  

\put(25, 100){\epsfig{file=media/simulated_human/simulated_confident_follower_test_1_safe_control_ourBRT20.png, width = 0.42\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
\put(0,  150){\epsfig{file=media/simulated_human/simulated_confident_follower_test_1_safe_control_ourBRT_latent_state20.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  

\put(25,  0){\epsfig{file=media/simulated_human/simulated_confident_follower_test_1_safe_control_ourBRT40.png, width = 0.42\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
\put(0,  50){\epsfig{file=media/simulated_human/simulated_confident_follower_test_1_safe_control_ourBRT_latent_state40.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  


% right side
\put(130, 200){\epsfig{file=media/simulated_human/simulated_less_confident_follower_test_3_safe_control_ourBRT3.png, width = 0.42\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}
\put(200,  250){\epsfig{file=media/simulated_human/simulated_less_confident_follower_test_3_safe_control_ourBRT_latent_state3.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}}


\put(130, 100){\epsfig{file=media/simulated_human/simulated_less_confident_follower_test_3_safe_control_ourBRT11.png, width = 0.42\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
\put(200,  150){\epsfig{file=media/simulated_human/simulated_less_confident_follower_test_3_safe_control_ourBRT_latent_state11.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  

\put(130,  0){\epsfig{file=media/simulated_human/simulated_less_confident_follower_test_3_safe_control_ourBRT25.png, width = 0.42\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
\put(200,  50){\epsfig{file=media/simulated_human/simulated_less_confident_follower_test_3_safe_control_ourBRT_latent_state25.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  


\put(25,290){(a-1)}
\put(25,190){(a-2)}
\put(25,90){(a-3)}
\put(125,290){(b-2)}
\put(125,190){(b-2)}
\put(125,90){(b-3)}

\end{picture}
\end{center}
%\vspace{-0.5cm}
\caption{(a-1)-(a-3) simulated human follower with high confidence; (b-1)-(b-3) simulated human with low confidence. Red: robot trajectory with full BRT as safety monitor.}
\label{fig: simulated human}
%\vspace{-0.4cm}
\end{figure}





% \begin{figure*}[thp!]
% \begin{center}
% \begin{picture}(600, 150)
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \put(25,  0){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control1.png, width = 0.25\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
% \put(0,  -5){\epsfig{file=media/simulated_human/simulated_confident_follower_latent_state45.png, width = 0.06\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  


% \put(170,  0){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control15.png, width = 0.25\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
% \put(145,  -5){\epsfig{file=media/simulated_human/simulated_confident_follower_latent_state45.png, width = 0.06\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 


% \put(315,  0){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control35.png, width = 0.25\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}}  
% \put(290,  -5){\epsfig{file=media/simulated_human/simulated_confident_follower_latent_state45.png, width = 0.06\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 


% \put(420,  60){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control_speed.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 

% \put(420,  10){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control_steering.png, width = 0.2\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 

% \end{picture}
% \end{center}
% %\vspace{-0.5cm}
% \caption{We can show: 1) put our BRT on real data and show the BRT shrinks to the true BRT 2) assume we use switching control strategy + a motion planner, what will happen if we use full BRT 3) what will happen if we use our BRT. The motion planner is a confounding variable. Need to emphasize that here we just demonstrate a potential use, any planner could work. If use full BRT, safe control introduces large lateral jerk}
% \label{fig:}
% %\vspace{-0.4cm}
% \end{figure*}


\begin{figure}[ht]
\begin{center}
\begin{picture}(300, 200)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(0,  0){\epsfig{file=media/traffic_data/roundabout_robot_planner.png, width = 0.5\linewidth, trim=3.5cm 2.5cm 0.5cm 3.5cm,clip}} 

\put(120,  60){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control_speed.png, width = 0.5\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 

\put(120,  10){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control_steering.png, width = 0.5\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 

\end{picture}
\end{center}
%\vspace{-0.5cm}
\caption{Left: Interaction trajectory between a human-driven car (purple) and a robot car (yellow). Red: full BRT; blue: Bayesian BRT; gray: least conservative BRT. \tr{Include BRT legends in the plot?} Blue line: robot trajectory with Bayesian BRT as safety monitor. Red line: robot trajectory with Full BRT as safety monitor. Right: robot speed history and angular velocity history.}
\label{fig: robot_vs_traffic_log}
%\vspace{-0.4cm}
\end{figure}



% \begin{figure}[ht]
% \begin{center}
% \begin{picture}(300, 200)
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \put(0,  0){\epsfig{file=media/traffic_data/highway_robot_planner.png, width = 0.9\linewidth, trim=5cm 0cm 0cm 1cm,clip}} 

% % \put(120,  60){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control_speed.png, width = 0.5\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 

% % \put(120,  10){\epsfig{file=media/traffic_data/traffic_data_test_3_safe_control_steering.png, width = 0.5\linewidth, trim=0cm 0cm 0cm 0cm,clip}} 

% \end{picture}
% \end{center}
% %\vspace{-0.5cm}
% \caption{}
% \label{fig:}
% %\vspace{-0.4cm}
% \end{figure}



\begin{figure}[ht]
\begin{center}
\begin{picture}(300, 200)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\put(0,  0){\epsfig{file=media/simulated_human/simulated_confident_follower_latent_state45.png, width = 0.15\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  

\put(40,  25){\epsfig{file=media/traffic_data/highway_traffic_data_test_2_safe_control1.png, width = 0.72\linewidth, trim=5cm 0cm 0cm 1cm,clip,angle =90}}  



\put(80,  0){\epsfig{file=media/traffic_data/highway_traffic_data_test_2_latent_state30.png, width = 0.15\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  

\put(120,  25){\epsfig{file=media/traffic_data/highway_traffic_data_test_2_safe_control30.png, width = 0.72\linewidth, trim=5cm 0cm 0cm 1cm,clip,angle =90}} 

\put(160,  0){\epsfig{file=media/traffic_data/highway_traffic_data_test_2_latent_state40.png, width = 0.15\linewidth, trim=0cm 0cm 0cm 0cm,clip}}  

\put(200,  25){\epsfig{file=media/traffic_data/highway_traffic_data_test_2_safe_control40.png, width = 0.72\linewidth, trim=5cm 0cm 0cm 1cm,clip,angle =90}} 


\end{picture}
\end{center}
%\vspace{-0.5cm}
\caption{}
\label{fig: robot_vs_traffic_log2}
%\vspace{-0.4cm}
\end{figure}


